Optimal Bounds on Approximation of Submodular and XOS Functions by Juntas

We investigate the approximability of several classes of real-valued functions by functions of a small number of variables ({\em juntas}). Our main results are tight bounds on the number of variables required to approximate a function $f:\{0,1\}^n \rightarrow [0,1]$ within $\ell_2$-error $\epsilon$ over the uniform distribution: 1. If $f$ is submodular, then it is $\epsilon$-close to a function of $O(\frac{1}{\epsilon^2} \log \frac{1}{\epsilon})$ variables. This is an exponential improvement over previously known results. We note that $\Omega(\frac{1}{\epsilon^2})$ variables are necessary even for linear functions. 2. If $f$ is fractionally subadditive (XOS) it is $\epsilon$-close to a function of $2^{O(1/\epsilon^2)}$ variables. This result holds for all functions with low total $\ell_1$-influence and is a real-valued analogue of Friedgut's theorem for boolean functions. We show that $2^{\Omega(1/\epsilon)}$ variables are necessary even for XOS functions. As applications of these results, we provide learning algorithms over the uniform distribution. For XOS functions, we give a PAC learning algorithm that runs in time $2^{poly(1/\epsilon)} poly(n)$. For submodular functions we give an algorithm in the more demanding PMAC learning model (Balcan and Harvey, 2011) which requires a multiplicative $1+\gamma$ factor approximation with probability at least $1-\epsilon$ over the target distribution. Our uniform distribution algorithm runs in time $2^{poly(1/(\gamma\epsilon))} poly(n)$. This is the first algorithm in the PMAC model that over the uniform distribution can achieve a constant approximation factor arbitrarily close to 1 for all submodular functions. As follows from the lower bounds in (Feldman et al., 2013) both of these algorithms are close to optimal. We also give applications for proper learning, testing and agnostic learning with value queries of these classes.

==> val-classes.tex <==
\section{Background on Submodular, XOS and Self-bounding functions}
\label{sec:classes}

In this section, we survey several related classes of set functions. The functions in these classes share some form of the property of ``forbidden complementarities" --- e.g., $f(\{a,b\})$ cannot be more than $f(\{a\}) + f(\{b\})$. However, there are several formalizations of this concept and the resulting classes have somewhat different properties. Since some of these classes evolved separately in different communities, the connections between them are not widely known. Therefore, we discuss briefly these classes of functions and their relationships. We also refer the reader to \cite{Vondrak10}, a short survey which discusses primarily the concentration properties of such functions.

%\subsubsection{Relationships between the classes of functions}

%Here, we discuss how the classes of functions relate to each other, and present some illustrative examples.

\noindent{\bf Linear functions.}
Linear (or additive) functions are functions in the form $f(S) = \sum_{i \in S} a_i$. This is the smallest class in the hierarchy that we consider here.

\noindent{\bf Submodular functions.}
A monotone submodular function can be viewed as a valuation on sets with the property of {\em diminishing returns}:
the marginal value of an element, $f_S(i) = f(S \cup \{i\}) - f(S)$, cannot increase if we enlarge the set $S$.
Non-monotone submodular functions play a role in combinatorial optimization, primarily as generalizations
of the {\em cut function} in a graph, $c(S) = |E(S, \bar{S})|$, which is known to be submodular. Another important subclass of monotone submodular functions is the class of {\em rank functions of matroids}: $r(S) = \max \{|I|: I \in \cI, I \subseteq S \}$, where $\cI$ is the family of independent sets in a matroid. In fact, it is known that a function of this type is submodular if and only if $\cI$ forms a matroid.

\noindent{\bf Fractionally subadditive functions (XOS).}
This class is broader than that of (nonnegative) monotone submodular functions (but does not contain non-monotone functions, since fractionally-subadditive functions are monotone by definition). For fractionally subadditive functions such that $f(\emptyset) = 0$,
there is an equivalent definition known as ``XOS":
$f$ is XOS iff $f(S) = \max_{i \in J} \sum_{j \in S} w_{ij}$ where $w_{ij} \geq 0$.

It is instructive to consider again the example of rank functions: $r(S) = \max \{|I|: I \in \cI, I \subseteq S \}$. As we mentioned,
$r(S)$ is submodular exactly when $\cI$ forms a matroid. In contrast, $r(S)$ is XOS for {\em any down-closed} set system $\cI$ (satisfying $A \subset B \in \cI \Rightarrow A \in \cI$;
this follows from an equivalent formulation of a rank function for down-closed set systems, $r(S) = \max \{ |S \cap I|: I \in \cI\}$). In this sense, XOS is a significantly broader class than submodular functions. Another manifestation of this fact is that optimization problems like $\max \{f(S): |S| \leq k\}$ admit constant-factor approximation algorithms using polynomially many {\em value queries} to $f$ when $f$ is submodular, but no such algorithms exist for XOS functions.

\noindent{\bf Subadditive functions.}
Subadditive functions are more general than submodular and fractionally subadditive functions.
In fact, subadditive functions are in some sense much less structured than fractionally subadditive  functions.
It is easy to verify that every function $f:2^N \rightarrow \{1,2\}$ is subadditive.
While submodular and fractionally subadditive functions satisfy ``dimension-free" concentration bounds, this is not true for subadditive functions (see \cite{Vondrak10} for more details).

\noindent{\bf Self-bounding functions.}
%Self-bounding functions also generalize ($1$-Lipschitz) fractionally subadditive functions. To subsume $1$-Lipschitz non-monotone submodular functions, it is sufficient to consider the slightly more general $2$-self-bounding functions - see \cite{Vondrak10}. The $1$-Lipschitz condition will not play a role in this paper, as we normalize functions to have values in the $[0,1]$ range.
Self-bounding functions satisfy {\em dimension-free concentration bounds}, based on the entropy method of Boucheron, Lugosi and Massart \cite{BoucheronLM:00}). Currently this is the most general class of functions known to satisfy such concentration bounds. The entropy method for self-bounding functions is general enough to rederive bounds such as Talagrand's concentration inequality.

A particular example of a self-bounding function (related to applications of Talagrand's inequality) is a function with the property of {\em small certificates}:
$f:X^n \rightarrow \ZZ_+$ has small certificates, if it is 1-Lipschitz and whenever $f(x) \geq k$, there is a set of coordinates $S \subseteq [n]$, $|S|=k$, such that if $y|_S = x|_S$, then $f(y) \geq k$. Such functions often arise in combinatorics, by defining $f(x)$ to equal the maximum size of a certain structure appearing in $x$. Another well-studied example self-bounding function are Rademacher averages which are widely used to measure the complexity of model classes in statistical learning theory \cite{Koltchinskii01,BartlettMendelson:02} (see \cite{Lugosi09} for a more detailed discussion and additional examples).

The definition of self-bounding functions is more symmetric than that of submodular: note that the definition does not change if we swap the meaning of $0$ and $1$ for any coordinate. This is a natural property to have in the setting of machine learning; the learnability of functions on $\zo^n$ should not depend on switching the meaning of $0$ and $1$ for any particular coordinate.



